Matching Cosmic Shear Analysis in Harmonic and Real Space

Recent cosmic shear analyses have exhibited discrepancies of up to $1\sigma$ between the inferred cosmological parameters when analyzing summary statistics in real space versus harmonic space. In this paper, we demonstrate the consistent measurement and analysis of cosmic shear two-point functions in harmonic and real space using the $i${\sc Master} algorithm. This algorithm provides a unified prescription to model the survey window effects and scale cuts in both real space (due to observational systematics) and harmonic space (due to model limitations), resulting in a matching estimation of the cosmic shear power spectrum from both harmonic and real space estimators. We show that the $i$\textsc{Master} algorithm gives matching results using measurements from the HSC Y1 mock shape catalogs in both real and harmonic space, resulting in matching inferences of $S_8=\sigma_8(\Omega_m/0.3)^{0.5}$. This method provides an unbiased estimate of the cosmic shear power spectrum, and $S_8$ inference that has a correlation coefficient of 0.997 between analyses using measurements in real space and harmonic space when $S_8$ is the only free parameter. We observe the mean difference between the two inferred $S_8$ values to be 0.0004 across noise-free mock realizations, far below the observed difference of 0.042 for the published HSC Y1 analyses and well below the statistical uncertainties. While the notation employed in this paper is specific to photometric galaxy surveys, the methods are equally applicable and can be extended to spectroscopic galaxy surveys, intensity mapping, and CMB surveys.

==> data.tex <==
\section{Data}
\label{sec:data}

\subsection{HSC Year 1 Shear Catalog}
The Hyper Suprime-Cam Subaru Strategic Program is a comprehensive imaging survey conducted using the 8.2 m Subaru Telescope and the Hyper Suprime-Cam wide-field camera (see \cite{2018PASJ...70S...4A} for survey design). The HSC survey consists of three layers: Wide, Deep, and UltraDeep. Each layer of the survey is observed in five broad-band filters ($grizy$) with a point source $5\sigma$ depth of $r \sim 26$ mag. It is this deep survey with excelling seeing (typical $i$-band seeing of $\sim0.59$ arcseconds) that allow HSC to measure cosmic shear signals up to higher redshifts with lower shape noise than other Stage III imaging surveys.

The HSC Year 1 shear catalog (HSC-Y1) is based on data from the HSC S16A internal data release, consisting of data taken between March 2014 to April 2016 with about 90 nights. A number of cuts have been made to construct a robust shape catalog for weak lensing analysis, including a conservative magnitude cut of $i < 24.5$, \xlrv{a resolution cut of $R_2>0.3$}, removing bad pixels, and masking regions of the sky around bright stars (see \cite{2018PASJ...70S..25M} for more details).



In this section, we describe the mock catalogs used to test our analysis
methods. We test the new analysis method using $579$ HSC Y1 mock shape catalogs
and verify that our new method produces the unbiased measurement of the
underlying true power spectrum. These mock catalogs are generated following the
method described in \cite{Shirasaki_2019} using the full-sky ray-tracing
$N$-body simulations \citep{raytracingTakahashi2017}. In short, real HSC
galaxies are populated to the simulated lensing field according to their
measured positions on the transverse plane, and their redshift is randomly
drawn from the estimated \textsc{MLZ} photometric redshift posterior, where
\textsc{MLZ} is a machine-learning code based on a self-organizing map for
photometric redshift (photo-$z$) inference. Therefore, the mock catalogs have the same
survey geometry as the real HSC Y1 data. These
realistic mocks are the perfect tests for our new analysis method as the HSC Y1
survey geometry is complex. As described in \cite{Shirasaki_2019}, the shear
catalog galaxies are divided into four tomographic redshift bins, in the
intervals $(0.3, 0.6], (0.6, 0.9], (0.9, 1.2],$ and $(1.2, 1.5]$, using the
``best" photo-z estimation by the \textsc{MLZ} algorithm.

The mock catalogs have galaxy positions in RA and Dec, true shear $\gamma_1$
and $\gamma_2$. We use the true shear value for our $F_\ell$ and $\xi$
measurements and use them to estimate the covariance matrix. We defer modeling
the covariance in \ref{sec:modeling_cov}.

% The HSC S16A data include photometric redshift (photo-$z$) estimates with a
% machine-learning code based on a self-organizing map (\textsc{MLZ}) and is
% estimated from the HSC five broadband photometry.

The mock catalogs adopt
a standard flat $\Lambda$CDM cosmological model with CDM density parameter
$\Omega_{c}=0.233$\,, the baryon density $\Omega_b=0.046$\,, the matter density
$\Omega_m=\Omega_c+\Omega_b=0.279$\,, the cosmological constant
$\Omega_\Lambda=0.721$\,, the Hubble parameter $h=0.7$\,, the amplitude of
density fluctuations $\sigma_8=0.82$\,, and the spectral index $n_s=0.97$\,.
\rachel{You adopt this because it's what was used for all of the mock catalog
realizations?  Or\dots?} \andy{Fixed.}

\rachel{My big-picture comment on this section is that you haven't described the HSC survey (briefly), referred to the survey definition paper, or given a reason why you think HSC is an interesting test case for this method.  You should also clarify just how much of the survey geometry is in the mocks, e.g., just the overall patch geometry or also bright star masks and other sources of complexity. I think a paragraph of such introductory material would be beneficial.}

